Clamped and sideband-resolved silicon optomechanical crystals

Optomechanical crystals (OMCs) are a promising and versatile platform for transduction between mechanical and optical fields. However, the release from the substrate used in conventional suspended OMCs also prevents heat-carrying noise phonons from rapidly leaking away. Thermal anchoring may be improved by attaching the OMCs directly to the substrate. Previous work towards such clamped, i.e. non-suspended, OMCs suffers from weak interaction rates and insufficient lifetimes. Here, we present a new class of clamped OMCs realizing -- for the first time -- optomechanical interactions in the resolved-sideband regime required for quantum transduction. Our approach leverages high-wavevector mechanical modes outside the continuum. We observe a record zero-point optomechanical coupling rate of $g_0/(2\pi) \approx 0.50$ MHz along with a sevenfold improvement in the single-photon cooperativity of clamped OMCs. Our devices operate at frequencies commonly used in superconducting qubits. This opens a new avenue using clamped OMCs in both classical and quantum communications, sensing, and computation through scalable mechanical circuitry that couples strongly to light.

==> commands.tex <==
\newcommand{\km}{k_\mathrm{m}}
\newcommand{\kp}{k_\mathrm{p}}
\newcommand{\ks}{k_\mathrm{s}}
\newcommand{\ko}{k_\mathrm{o}}
\newcommand{\op}{\omega_\mathrm{p}}
\newcommand{\os}{\omega_\mathrm{s}}
\newcommand{\om}{\omega_{\rm m}}
\newcommand{\oo}{\omega_{\rm o}}
\newcommand{\E}{\boldsymbol{E}}
\newcommand{\Ef}{\tilde{\boldsymbol{E}}_\mathrm{f}}
\newcommand{\Eb}{\tilde{\boldsymbol{E}}_\mathrm{b}}
\newcommand{\Q}{\boldsymbol{u}}
\newcommand{\Qf}{\tilde{\boldsymbol{u}}_\mathrm{f}}
\newcommand{\Qb}{\tilde{\boldsymbol{u}}_\mathrm{b}}
\newcommand{\kmf}{k_\mathrm{m,f}}
\newcommand{\kmb}{k_\mathrm{m,b}}
\newcommand{\kof}{k_\mathrm{o,f}}
\newcommand{\kob}{k_\mathrm{o,b}}
\renewcommand{\d}{\mathrm{d}}
\renewcommand{\r}{\boldsymbol{r}}

